You, the Web and Your Device: Longitudinal Characterization of Browsing Habits

Understanding how people interact with the web is key for a variety of applications, e.g., from the design of effective web pages to the definition of successful online marketing campaigns. Browsing behavior has been traditionally represented and studied by means of clickstreams, i.e., graphs whose vertices are web pages, and edges are the paths followed by users. Obtaining large and representative data to extract clickstreams is however challenging. The evolution of the web questions whether browsing behavior is changing and, by consequence, whether properties of clickstreams are changing. This paper presents a longitudinal study of clickstreams in from 2013 to 2016. We evaluate an anonymized dataset of HTTP traces captured in a large ISP, where thousands of households are connected. We first propose a methodology to identify actual URLs requested by users from the massive set of requests automatically fired by browsers when rendering web pages. Then, we characterize web usage patterns and clickstreams, taking into account both the temporal evolution and the impact of the device used to explore the web. Our analyses precisely quantify various aspects of clickstreams and uncover interesting patterns, such as the typical short paths followed by people while navigating the web, the fast increasing trend in browsing from mobile devices and the different roles of search engines and social networks in promoting content. Finally, we contribute a dataset of anonymized clickstreams to the community to foster new studies (anonymized clickstreams are available to the public at http://bigdata.polito.it/clickstream).

==> lib/chronosys/chronosyschr.tex <==
% This is is the main file of the `chronosys' package, with all the principal code.
%
% The maintener of this work is Mathieu Long.
% email : mlong.tex@hotmail.fr
% the `chronosys' package consists in the 9 files :
%  -- `docchronosys_en.tex' and `docchronosys_en.pdf' (english manual)
%  -- `docchronosys_fr.tex' and `docchronosys_fr.pdf' (french manual)
%  -- README
%  -- `chronosys.tex' (file for plain TeX)
%  -- `chronosyschr.tex' (main file of the `chronosys' package)
%  -- `chronosys.sty' (file for LaTeX)
%  -- `x-chronosys.tex' (file for ConTeXt)
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
% 
% The Current Maintainer of this work is Mathieu Long.
%
\expandafter\ifx\csname chronosys @\endcsname\relax\else\immediate\write16{Le fichier a deja ete charge}\endinput\fi
\ifx\numexpr\UNDEFINED\immediate\write16{Desole, mais ce fichier utilise les primitives E-TeX, vous ne pouvez pas utiliser le moteur TeX.}\endinput\fi
\expandafter\edef\csname chronosys @\endcsname{\the\catcode`\@}%
\catcode`\@=11%
\catcode`\!=11%
\def\chron@sysversion{1.2}%
%
\newhelp\chrhelpmessage{Contactez l'auteur par mail.}%
\newhelp\chrerrormessage{La commande a deja ete definie.}%
\def\error!message{\errhelp{\the\chrhelpmessage}\errmessage{\the\chrerrormessage}} %
%
\def\!chrverif#1#2{\ifdefined#2\expandafter\error!message \fi #1#2}%
%
%Commandes utilis\'ees 
%
%
\def\!gobblethree#1#2#3{}%
\def\!gobble#1{}%
\ifdefined\@ifnextchar %LATEX
  \def\:{\let\ifnexttoken\@ifnextchar}\expandafter\:
\else 
  \ifdefined\doifnextcharelse %CONTEXT
    \def\:{\let\ifnexttoken\doifnextcharelse}\expandafter\:
  \else 
    \long\def\@ifnextchar#1#2#3{%
      \let\reserved@d=#1%
      \def\reserved@a{#2}%
      \def\reserved@b{#3}%
      \futurelet\@let@token\@ifnch}%
      \let\kernel@ifnextchar\@ifnextchar
      \def\@ifnch{%
        \ifx\@let@token\@sptoken
          \let\reserved@c\@xifnch
        \else
          \ifx\@let@token\reserved@d
            \let\reserved@c\reserved@a
          \else
            \let\reserved@c\reserved@b
          \fi
        \fi
    \reserved@c}%
\def\:{\let\@sptoken= }\: % this makes \@sptoken a space token
\def\:{\@xifnch}\expandafter\def\: {\futurelet\@let@token\@ifnch}%
\let\ifnexttoken\@ifnextchar
\fi\fi
%
\newif\if!chronearg \newif\if!chrtwoarg 
\!chrverif\def\!chrtraiteoneargument#1{\ifnexttoken[{\!chroneargtrue#1}{\!chroneargfalse#1[]}}%
%
\!chrverif\def\!chrtraitetwoargument#1{\let\todoafterarg#1%
\ifnexttoken[{\!chroneargtrue\savefirsttwoarg}{\!chroneargfalse\!chrtwoargfalse#1[][]}}%
\!chrverif\def\savefirsttwoarg[#1]{\ifnexttoken[{\!chrtwoargtrue \todoafterarg[#1]}{\!chrtwoargfalse \todoafterarg[#1][]}}%
%
\!chrverif\def\!chrtraitingargvirgule#1#2{\def\!tr@itintargvirgule{#2}\!chrtr@itingargvirgule#1,\end}%
\!chrverif\def\!chrtr@itingargvirgule#1,{%
\!chrdotraiteargvirgule#1,=\end,\ifnexttoken\end \!gobble \!chrtr@itingargvirgule}%
\!chrverif\def\!chrdotraiteargvirgule#1=#2,{%
\ifx \end#2\relax
\else \!chrdotr@iteargvirgule#1=#2,\expandafter\!gobblethree
\fi}%
\!chrverif\def\!chrdotr@iteargvirgule#1=#2,{%
\ifcsname \!tr@itintargvirgule#1\endcsname
 \expandafter\def\csname \!tr@itintargvirgule#1\endcsname{#2}%
\else \immediate\write16{chronosys : option #1 ligne \number\inputlineno\space non reconnue, impossible de lui affecter la valeur #2}%
\fi }%
%
%STARTCHRONOLOGY
%
\!chrverif\def\startchronology{\!chrtraiteoneargument\dostartchronology}%
%
%OPTIONS DE STARTCHRONOLOGY
%
\!chrverif\def\!chrdefaultstartyear{0}\!chrverif\def\!chrdefaultstopyear{\the\year}\!chrverif\def\!chrdefaultwidth{\the\hsize}%
\!chrverif\def\!chrdefaultheight{0.7pc}\!chrverif\def\!chrdefaultdates{true}\!chrverif\def\!chrdefaultarrow{true}% 
\!chrverif\def\!chrdefaultarrowwidth{0.1\!chrwidth}\!chrverif\def\!chrdefaultdateselevation{20pt}%
\!chrverif\def\!chrdefaultarrowheight{\!chrheight}\!chrverif\def\!chrdefaultcolor{black}\!chrverif\def\!chrdefaultarrowcolor{\!chr@color}%
\!chrverif\def\!chrdefaultdatesstyle{}\!chrverif\def\!chrdefaultstartdate{true}\!chrverif\def\!chrdefaultstopdate{true}% 
\!chrverif\def\!chrdefaultbox{false}\!chrverif\def\!chrdefaultalign{center}%
%
\!chr@verif\newdimen\!chrheight \!chr@verif\newif\if!chrdates \!chr@verif\newif\if!chrarrow \!chr@verif\newcount\!chrstartyear
\!chr@verif\newcount\!chrstopyear \!chr@verif\newdimen\!chrwidth \!chr@verif\newdimen\!chrarrowwidth \!chr@verif\newdimen\!chrarrowheight 
\!chr@verif\newbox\!chrflechebox 
\!chr@verif\newdimen\!chr!realwidth \!chr@verif\newdimen\!chr!unitperyear
\!chr@verif\newif\if!chrstartdate \!chr@verif\newif\if!chrstopdate \!chr@verif\newdimen\!chrdateselevation \!chr@verif\newif\if!chrbox
%
\!chrverif\def\!chr!periodeschwarzodergrau{\def\!chr!stringtest{black}%
\ifx\!chr@color\!chrstringtest
  \def\!chr!periodeschwarzodergr@u{gray}%
\else
  \def\!chr!periodeschwarzodergr@u{black}%
\fi}%
%
%
\!chr@verif\newdimen\!chrskipbefore
\!chr@verif\newdimen\!chrskipafter
%
\!chrverif\def\!chrdefaultoptions{startyear=\!chrdefaultstartyear, stopyear=\!chrdefaultstopyear,
startdate=\!chrdefaultstartdate, stopdate=\!chrdefaultstopdate,
height=\!chrdefaultheight, width=\!chrdefaultwidth, dates=\!chrdefaultdates, arrow=\!chrdefaultarrow,
arrowwidth=\!chrdefaultarrowwidth, arrowheight=\!chrdefaultarrowheight, color=\!chrdefaultcolor,
arrowcolor=\!chrdefaultarrowcolor, datesstyle=\!chrdefaultdatesstyle, dateselevation=\!chrdefaultdateselevation,
box=\!chrdefaultbox, align=\!chrdefaultalign}%
%
\!chrverif\def\!chr@startyear{}\!chrverif\def\!chr@startdate{}%
\!chrverif\def\!chr@stopyear{}\!chrverif\def\!chr@stopdate{}%
\!chrverif\def\!chr@height{}\!chrverif\def\!chr@width{}%
\!chrverif\def\!chr@dates{true}%
\!chrverif\def\!chr@arrow{}\!chrverif\def\!chr@arrowwidth{}\!chrverif\def\!chr@arrowheight{}% 
\!chrverif\def\!chr@color{}% 
\!chrverif\def\!chr@arrowcolor{}\!chrverif\def\!chr@datesstyle{}% 
\!chrverif\def\!chr@dateselevation{}%
\!chrverif\def\!chr@box{}\!chrverif\def\!chr@align{}%
%
%DOSTARTCHRONOLOGY
%
\!chrverif\def\dostartchronology[#1]{\begingroup\parindent\z@\par
\global\!chrskipafter\z@
\global\!chrskipbefore\z@
\expandafter\expandafter\expandafter\!chrtraitingargvirgule\expandafter{\!chrdefaultoptions}{!chr@}%
\if!chronearg \!chrtraitingargvirgule{#1}{!chr@}\fi 
\!chrheight\!chr@height   \!chrstartyear\!chr@startyear 
\!chrstopyear\!chr@stopyear    \!chrwidth\!chr@width %
\csname !chrdates\!chr@dates\endcsname \csname !chrarrow\!chr@arrow\endcsname 
\csname !chrstartdate\!chr@startdate\endcsname  \csname !chrbox\!chr@box\endcsname 
\csname !chrstopdate\!chr@stopdate\endcsname \!chrarrowwidth\!chr@arrowwidth 
\!chrarrowheight\!chr@arrowheight \!chrdateselevation\!chr@dateselevation%
\!chr!periodeschwarzodergrau%
\dostartchronologyfinal}%
%
\!chrverif\def\dostartchronologyfinal{%
\unless\if!chrarrow
  \!chrarrowwidth\z@\relax \!chrarrowheight\z@
\fi
\!chr!realwidth\dimexpr\!chrwidth-\!chrarrowwidth\relax
\ifdim\!chr!realwidth<0pt\relax
  \advance\!chrwidth\dimen@ 
  \advance\!chrarrowwidth-\!chr!realwidth 
  \!chr!realwidth\z@
\fi 
\dimen@\dimexpr\!chrheight-\!chrarrowheight\relax  
\dimen@ii\dimen@\relax
\ifdim\dimen@ii>0pt\relax
  \dimen@ii\z@
\fi
\dimen@i\dimexpr\!chrheight-\dimen@ii+\!chrdateselevation\relax
% % %AFFICHAGE DE LA FRISE
\setbox\!chrflechebox\hbox{%
  \if!chrdates
    \if!chrstartdate\raise\dimen@i\relax % %
      \hbox to\z@{\hss\!chr@datesstyle{\the\!chrstartyear}\hss}%
    \fi
  \fi%
%  \!chrstarttikzpicture\!chrfilldraw[color=\!chr@color](0,0)--(\the\!chr!realwidth,0)--(\the\!chr!realwidth,\the\!chrheight)--(0,\the\!chrheight)--cycle;
%  \if!chrbox
%    \!chrdraw[color=black](-0.4pt,-0.4pt)--(\the\!chr!realwidth+0.4pt,-0.4pt)--(\the\!chr!realwidth+0.4pt,\the\!chrheight+0.4pt)--(-0.4pt,\the\!chrheight)--cycle;
%  \fi %
%  \if!chrarrow
%    \ifx\!chr@color\!chr@arrowcolor
%    \else \!chrdraw[color=\!chr!periodeschwarzodergr@u](\the\!chr!realwidth,0)--(\the\!chr!realwidth,\the\!chrheight);
%    \fi
%  \fi
%  \!chrstoptikzpicture %
  \begingroup{%
  \!chrusecolor{\!chr@color}%
  \vrule width\!chr!realwidth height\!chrheight depth\z@\relax \kern-\!chr!realwidth\relax
  \if!chrbox
    \!chrusecolor{black}%
    \hbox to\z@{\vrule width\!chr!realwidth height0.4pt\relax\hss}%
    \raise\!chrheight\hbox to\z@{\vrule width\!chr!realwidth height0.4pt\relax\hss}%
    \vrule height\!chrheight depth\z@\relax\kern-0.4pt\relax
    \kern\!chr!realwidth \vrule height\!chrheight\relax\kern-0.4pt\relax
    \kern-\!chr!realwidth
  \fi
  %\if!chrarrow
  %\fi
  \kern\!chr!realwidth
  }%
  \endgroup
  \if!chrdates
    \if!chrstopdate
      \raise\dimen@i\hbox to\z@{\hss\!chr@datesstyle{\the\!chrstopyear}\hss}%
    \fi
  \fi%
%
  \if!chrarrow
    \raise0.5\dimen@\hbox{%
      \!chrstarttikzpicture
      \!chrfilldraw[color=\!chr@arrowcolor](0,0.5*\the\!chrarrowheight-0.4pt)--(\the\!chrarrowwidth,0)--(0,-0.5*\the\!chrarrowheight)--cycle;
      \if!chrbox
        \!chrdraw[color=black](-0.4pt,0.5*\the\!chrarrowheight+0.4pt)--(\the\!chrarrowwidth+0.4pt,0)--(-0.4pt,-0.5*\the\!chrarrowheight-0.4pt)--cycle;
      \fi
      \!chrstoptikzpicture
      \edef\@@string@a{\!chr@color}%
      \edef\@@string@b{\!chr@arrowcolor}%
      \ifx\@@string@a\@@string@b
      \else
        {\!chrusecolor{\!chr!periodeschwarzodergr@u}%
        \kern-\!chrarrowwidth\kern-0.2pt\relax \hbox to\z@{\vrule height\dimexpr(\!chrarrowheight-\!chrheight)/2 + \!chrheight\relax depth\dimexpr(\!chrheight-\!chrarrowheight)/2\relax\hss}% 
        \kern\!chrarrowwidth\kern-0.2pt\relax}%
      \fi
    }%
  \fi}%
  \count@\numexpr\!chrstopyear-\!chrstartyear\relax
  \ifnum\count@<0\relax
    \immediate\write16{Erreur avec les dates donn\'ees}%
  \fi 
  \!chr!unitperyear\dimexpr\!chr!realwidth/\count@\relax}%
%
%
\!chrverif\def\setupchronology#1{\!chrtraitingargvirgule{#1}{!chrdefault}}%
%
%PERIODES
%
\!chr@verif\newcount\!chr!periodecolornum\!chr@verif\newcount\!chr!starttingtraitement \!chr@verif\newdimen\!chr!dimentraitement
\!chr@verif\newdimen\!chrperiodtextdepth \!chrverif\def\!chrperiodedefaulttextdepth{15pt}% 
\!chr@verif\newif\if!chrperioddates  \!chr@verif\newif\if!chrperiodbox
\!chr@verif\newif\if!chrperiodstartdate \!chr@verif\newif\if!chrperiodstopdate \!chrverif\def\!chrperiodedefaultstartdate{true}
\!chr@verif\newif\if!chrperiodifcolorbox 
\!chr@verif\newdimen\!chrperioddateselevation 
\!chr@verif\newdimen\!chrperiodeventtextwidth 
\!chr@verif\newdimen\!chrperiodbottomdepth \!chr@verif\newdimen\!chrperiodtopheight
%
%alternance des couleurs
\!chr@verif\newcount\!chrperiodecoloralternancetotalnum
\!chrverif\def\!chrperiodedefaultcolor{\chronoperiodcolor}%
\!chrverif\def\!chrperiodedefa@@ultcolor{\chronoperiodcolor}%
\!chrverif\def\!chrperiodedef@ultcolor{\!chrperiodedefaultcolor}%
\!chrverif\def\chronoperiodcolor{\ifcase\!chr!periodecolornum blue\or red\or cyan\or purple\or yellow\fi}%
\!chrperiodecoloralternancetotalnum5%
\!chrverif\def\!chr!periodecolor{\edef\!chrperiodedef@ultcolor{\!chrperiodedefaultcolor}%
  \ifx\!chrperiodedefaultcolor\!chrperiodedefa@@ultcolor
    \ifx\!chrperiodedef@ultcolor\!chr@color
      \!chr!periodecoloradvance\!chr!periodecolor 
    \fi
  \fi}%
\!chrverif\def\!chr!periodecoloradvance{\global\advance\!chr!periodecolornum\@ne\relax
\ifnum\!chr!periodecolornum=\!chrperiodecoloralternancetotalnum\relax\global\!chr!periodecolornum\z@\fi}%
%
\!chrverif\def\restartchronoperiodecolor{\!chrtraiteoneargument\dorestartchronoperiodecolor}%
\!chrverif\def\dorestartchronoperiodecolor[#1]{%
\if!chronearg 
  \def\@@string@a{#1}%
  \!chr!periodecolornum\z@ %
  \dorestartchronoperiodecolor@ux
\else
  \!chr!periodecolornum\z@
\fi}%
\!chrverif\def\dorestartchronoperiodecolor@ux{\edef\@@string@b{\chronoperiodcolor}%
\ifnum\!chr!periodecolornum<\!chrperiodecoloralternancetotalnum
  \unless\ifx\@@string@a\@@string@b
    \global\advance\!chr!periodecolornum\@ne 
    \dorestartchronoperiodecolor@ux
  \fi
\else\global\!chr!periodecolornum\z@\fi}%
%
\!chrverif\def\chronoperiodecoloralternation#1{%
\def\@@string@s{\ifcase\!chr!periodecolornum}%
\!chrperiodecoloralternancetotalnum\z@\!chr!chronoperiodecoloralternance#1,\end \let\chronoperiodcolor\@@string@s
\!chr!periodecolornum\z@}%
%
\!chrverif\def\!chr!chronoperiodecoloralternance#1,{\advance\!chrperiodecoloralternancetotalnum\@ne
\expandafter\def\expandafter\@@string@s\expandafter{\@@string@s#1}%
\ifnexttoken\end {\expandafter\def\expandafter\@@string@s\expandafter{\@@string@s\fi}\!gobble}%
{\expandafter\def\expandafter\@@string@s\expandafter{\@@string@s\or}\!chr!chronoperiodecoloralternance}}%
%
%
\!chrverif\def\!chr@periodtextdepth{}\!chrverif\def\!chr@perioddates{}%
\!chrverif\def\!chr@periodcolor{}\!chrverif\def\!chr@perioddatesstyle{}%
\!chrverif\def\!chr@periodstartdate{}\!chrverif\def\!chr@periodstopdate{}%
\!chrverif\def\!chr@periodtextstyle{}%
\!chrverif\def\!chr@perioddateselevation{}%
\!chrverif\def\!chr@periodifcolorbox{}\!chrverif\def\!chr@periodcolorbox{}%
\!chrverif\def\!chr@periodbottomdepth{}\!chrverif\def\!chr@periodtopheight{}%
\!chrverif\def\!chr@periodbox{}\!chrverif\def\!chr@periodtextwidth{}%
%
\!chrverif\def\!chreventdefaulttesttextwidth{\relax}%
%
%DOCHRONOPERIODE
%
%
\!chrverif\def\dochronoperiode[#1]#2#3#4{%
\!chr!periodecolor %alternance automqatique des couleurs
\if!chronearg \!chrtraitingargvirgule{#1}{!chr@period}\fi
% % %
\!chrperiodtextdepth\!chr@periodtextdepth \!chrperiodtopheight\!chr@periodtopheight
\!chrperiodbottomdepth\!chr@periodbottomdepth
\csname !chrperioddates\!chr@perioddates\endcsname \csname !chrperiodstartdate\!chr@periodstartdate\endcsname 
\csname !chrperiodstopdate\!chr@periodstopdate\endcsname \csname !chrperiodifcolorbox\!chr@periodifcolorbox\endcsname
\csname !chrperiodbox\!chr@periodbox\endcsname
\ifx\!chr@periodtextwidth\!chreventdefaulttesttextwidth
	\!chrperiodeventtextwidth=-1pt%
\else
	\!chrperiodeventtextwidth=\!chr@periodtextwidth%
\fi
\!chrperioddateselevation\!chr@perioddateselevation 
\advance\!chrperioddateselevation 1.25\!chrheight\relax
% % %On s'assure que les dates sont biebn dans l'intervalle
\ifnum#2>\numexpr\!chrstartyear-1\relax
\ifnum#2<\numexpr\!chrstopyear+1\relax
\ifnum#3<\numexpr\!chrstopyear+1\relax 
\ifnum#3>\numexpr\!chrstartyear-1\relax
\count@\numexpr#3-#2\relax
% % %Et que la seconde est post\'erieure \`a la pr\'emi\`ere
\ifnum\count@>\z@\relax
% %
\!chr!starttingtraitement\numexpr#2-\!chrstartyear\relax\dimen@\dimexpr\count@\!chr!unitperyear\relax
\!chr!dimentraitement\dimexpr\!chr!starttingtraitement\!chr!unitperyear\relax
% %AFFICHAGE
\dimen@i\wd\!chrflechebox
\setbox\!chrflechebox\hbox{%
  \unhbox\!chrflechebox\kern-\dimen@i\kern\!chr!dimentraitement
  \lower\dimexpr\!chrperiodtextdepth-\!chrperiodbottomdepth\relax\hbox to\z@{%
    \ifdim\!chrperiodeventtextwidth < \z@ \hbox to\dimen@{%
      	\hss \if!chrperiodifcolorbox\expandafter\!chrperiodcolorbox\fi{\!chr@periodtextstyle{#4}}\hss
    	}%
    \else
       \setbox\z@\hbox to\dimen@{\hss\vbox{%
       \hsize\!chrperiodeventtextwidth {\!chr@periodtextstyle{#4}}
       }\hss}%
       \dimen@i\wd\z@
       \dimen@ii\dimexpr\ht\z@+\dp\z@\relax
       \lower\dimexpr\dimen@ii-10pt\relax\hbox to\dimen@{%
          \hss\setbox\z@\hbox{%
           \vbox{%
            \hsize\!chrperiodeventtextwidth\relax\!chr@periodtextstyle{#4}%
            \vskip1pt
           }%
          }%
          \dimen@i\dimexpr\wd\z@+4pt\relax
          \dimen@ii\dimexpr\ht\z@+\dp\z@+2pt\relax
          \setbox\z@\hbox to\z@{%
          \hss\begingroup{\!chrusecolor{\!chr@periodcolorbox}\vrule height\dimen@ii width\dimen@i depth2pt}\endgroup\kern-\dimen@i\kern2pt\relax%
                     \box\z@\hss
          }%
          \box\z@\hss
       }%
    \fi
    \hss
  }%
  \if!chrperioddates
    \if!chrperiodstartdate
      \raise\dimexpr\!chrperioddateselevation +(\!chrperiodtopheight-\!chrheight)\relax 
      \hbox to\z@{%
        \hss\!chr@perioddatesstyle{#2}\hss
      }%
    \fi
  \fi 
  \raise\!chrperiodbottomdepth \hbox{%
    \begingroup {\!chrusecolor{\!chr@periodcolor}%
       \dimen@i\dimexpr\!chrperiodtopheight-\!chrperiodbottomdepth\relax%
       \vrule width\dimen@ height\dimen@i depth\z@\kern-\dimen@%
%       \!chrusecolor{black}%
%       \raise\dimen@i\hbox to\z@{\vrule height0.1pt depth0.3pt width\dimen@\hss}%
%       \hbox to\z@{\vrule height0.1pt depth0.3pt width\dimen@\hss}%
    }\endgroup%%
    \begingroup{%
    \dimen@i\dimexpr\!chrperiodtopheight-\!chrperiodbottomdepth\relax%
    \!chrusecolor{\!chr!periodeschwarzodergr@u}%
    \kern-0.2pt\relax\vrule height\dimen@i width0.4pt\relax  \kern-0.2pt\relax%
    \kern\dimen@\relax
    \kern-0.2pt\relax\vrule height\dimen@i width0.4pt\relax  \kern-0.2pt\relax
    \kern-\dimen@\relax
    }%
    \endgroup
    \begingroup{%
    \!chrusecolor{black}
    \if!chrbox
      \lower 0.2pt\hbox to\z@{\vrule width\dimen@\hss}%
    \fi
    \if!chrperiodbox
      \raise \!chrperiodbottomdepth \hbox to\z@{\vrule width\dimen@\hss}%
      \raise \!chrperiodtopheight \hbox to\z@{\vrule width\dimen@\hss}%
    \fi
    }%
    \endgroup
    \kern\dimen@\relax
  }%
  \if!chrperioddates
    \if!chrperiodstopdate
      \raise\dimexpr\!chrperioddateselevation+(\!chrperiodtopheight-\!chrheight)\relax
      \hbox to\z@{%
        \hss \!chr@perioddatesstyle{#3}\hss
      }%
    \fi
  \fi
}%
\!chr!periodecoloradvance
\fi\fi\fi\fi\fi}%
%
%
\!chrverif\def\setupchronoperiode{\def\@@string@a{periode}\!chrtraiteoneargument\dosetupchronoeventandperiode}%
%
%EVENTS
%
%
\!chr@verif\newif\if!chreventspecifiedday\!chr@verif\newif\if!chreventspecifiedmonth \!chr@verif\newif\if!chreventbarre
\!chr@verif\newif\if!chreventdate  \!chr@verif\newif\if!chreventmark
\!chr@verif\newif\if!chreventifcolorbox \!chr@verif\newif\if!chreventconversionmonth 
\!chr@verif\newdimen\!chreventmarkdepth \!chr@verif\newif\if!chreventyear \!chr@verif\newdimen\!chreventiconheight
 \!chrverif\def\!chreventdefaultbarre{true}%
\!chrverif\def\!chreventdefaulticon{}%
\!chrverif\def\!chreventdefaultmarkdepth{10pt}%
\!chrverif\def\!chreventdefaulttextstyle{}%
%
%
%
\!chrverif\def\!chreventevalspecification#1{\count@\z@\relax\!chreventev@lspecification#1/\end}%
\!chrverif\def\!chreventev@lspecification#1/{\advance\count@\@ne\relax\expandafter\def\csname
!chreventspecifiedargument\number\count@\endcsname{#1}\ifnexttoken\end \!gobble \!chreventev@lspecification}%
%
\!chrverif\def\chron@selectmonth#1{\ifcase#1\or janvier\or f\'evrier\or mars\or avril\or mai\or juin\or juillet\or ao\^ut\or septembre\or octobre\or novembre\or d\'ecembre\fi}%
%
\!chrverif\def\!chr@eventbarre{}\!chrverif\def\!chr@eventicon{}\!chrverif\def\!chr@eventmarkdepth{}%
\!chrverif\def\!chr@eventtextstyle{}\!chrverif\def\!chr@eventmark{}%
\!chrverif\def\!chr@eventdate{}\!chrverif\def\!chr@eventdatesseparation{}%
\!chrverif\def\!chr@eventconversionmonth{}\!chrverif\def\!chr@eventdatestyle{}%
\!chrverif\def\!chr@eventdatesstyle{}\!chrverif\def\!chr@eventyear{}\!chrverif\def\!chr@eventiconheight{}%
\!chrverif\def\!chr@eventifcolorbox{}\!chrverif\def\!chr@eventcolorbox{}%.
\!chrverif\def\!chr@eventtextwidth{}%
% 
\!chr@verif\newif\if!chreventlocationup
%
%
%DOCHRONOEVENT
%
%
\!chrverif\def\dochronoevent[#1]#2#3{%
\if!chronearg \!chrtraitingargvirgule{#1}{!chr@event}\fi
% % %
\csname !chreventbarre\!chr@eventbarre\endcsname 
\csname !chreventmark\!chr@eventmark\endcsname 
\csname !chreventdate\!chr@eventdate\endcsname
\csname !chreventconversionmonth\!chr@eventconversionmonth\endcsname 
\csname !chreventyear\!chr@eventyear\endcsname
\csname !chreventifcolorbox\!chr@eventifcolorbox\endcsname
\!chreventmarkdepth\!chr@eventmarkdepth 
\!chreventiconheight\!chr@eventiconheight
\ifx\!chr@eventtextwidth\!chreventdefaulttesttextwidth 
   \!chrperiodeventtextwidth=-1pt%
\else \!chrperiodeventtextwidth\!chr@eventtextwidth
\fi
\ifdim\!chreventmarkdepth<\z@\relax
  \!chreventlocationuptrue
\else
  \!chreventlocationupfalse
\fi
% % % Evaluation de la precision de la date de l'evenement
\!chreventevalspecification{#2}%
\ifnum\count@<4\relax
  \ifcase\count@
    \or \!chreventspecifieddayfalse\!chreventspecifiedmonthfalse 
        \edef\!chreventyear{\csname !chreventspecifiedargument1\endcsname}%
    \or \!chreventspecifieddayfalse\!chreventspecifiedmonthtrue
        \edef\!chreventyear{\csname !chreventspecifiedargument2\endcsname}%
        \edef\!chreventmonth{\csname !chreventspecifiedargument1\endcsname}%
    \or \!chreventspecifieddaytrue\!chreventspecifiedmonthtrue
        \edef\!chreventyear{\csname !chreventspecifiedargument3\endcsname}%
        \edef\!chreventmonth{\csname !chreventspecifiedargument2\endcsname}%
        \edef\!chreventday{\csname !chreventspecifiedargument1\endcsname}%
  \fi %
% %On s'assure que les dates sont bien comprises dans les bornes
\ifnum\!chreventyear>\numexpr\!chrstartyear-1\relax
\ifnum\!chreventyear<\numexpr\!chrstopyear+1\relax
      \if!chreventspecifiedmonth
        \if!chreventspecifiedday 
          \count@\numexpr\!chreventday+\!chreventmonth*30\relax
        \else %
          \count@\numexpr\!chreventmonth*30\relax
        \fi
      \else \count@\z@
      \fi %
      \!chr!dimentraitement\dimexpr(\!chr!unitperyear)/365*\count@\relax%
     \count@\numexpr\!chreventyear-\!chrstartyear\relax 
     \advance\!chr!dimentraitement\dimexpr\count@\!chr!unitperyear\relax
% % % Affichage
     \dimen@i\wd\!chrflechebox
     \setbox\!chrflechebox\hbox{%
       \unhbox\!chrflechebox\kern-\dimen@i\kern\!chr!dimentraitement
       \if!chreventbarre
        \begingroup{%
        \!chrusecolor{black}%
        \kern-0.4pt\relax\vrule width0.4pt height\!chrheight depth\z@\relax
        }%
        \endgroup
       \fi
       \kern-0.4pt\raise\!chreventiconheight \hbox to\z@{\hss\!chr@eventicon\hss}%
       \lower\dimexpr\!chreventmarkdepth+2pt\relax
       \hbox to\z@{%
         \vbox to\z@{%
           \if!chreventlocationup\relax\vss\fi
           \if!chreventdate\hbox to\z@{%
             \hss \if!chreventifcolorbox \expandafter\!chreventcolorbox\fi
             {\!chr@eventdatestyle{%
%               \if!chreventspecifiedday %
%                 {\!chr@eventdatesstyle{\!chreventday}}\!chr@eventdatesseparation
%               \fi
             {\!chr@eventdatesstyle{%
%               \if!chreventspecifiedmonth 
%                 \if!chreventconversionmonth\expandafter \chron@selectmonth
%                 \fi 
%                 \!chreventmonth
%               \fi
               }%
             }%
             \if!chreventspecifiedmonth\if!chreventyear \!chr@eventdatesseparation\fi\fi 
             \if!chreventyear{\!chr@eventdatesstyle{\!chreventyear}}\fi%
             }}%
             \hss
           }%
           \fi
           \ifdim\!chrperiodeventtextwidth > \z@ 
             \hbox to\z@{%
               \hss\setbox\z@\hbox{%
                 \vbox{%
                   \hsize\!chrperiodeventtextwidth\relax\!chr@eventtextstyle{#3}%
                   \vskip1pt\relax
                 }%
               }%
               \dimen@i\dimexpr\wd\z@+4pt\relax
               \dimen@ii\dimexpr\ht\z@+\dp\z@+2pt\relax
               \setbox\z@\hbox to\z@{%
                 \hss\begingroup{\!chrusecolor{\!chr@eventcolorbox}\vrule height\dimen@ii width\dimen@i depth2pt\relax}\endgroup \kern-\dimen@i\kern2pt\relax%
                 \box\z@\hss
               }%
               \box\z@
             }%
           \else 
             \hbox to\z@{%
               \hss\if!chreventifcolorbox\expandafter\!chreventcolorbox\fi{%
               \!chr@eventtextstyle{#3}}\hss
             }%
           \fi 
           \unless\if!chreventlocationup\relax\vss\fi
         }%
       }%
       \if!chreventmark
         \if!chreventlocationup\relax
         %\!chrstarttikzpicture \!chrdraw(0,0)--(0,\the\!chreventmarkdepth+5pt);\!chrstoptikzpicture
           \vrule height\dimexpr-\!chreventmarkdepth-5pt\relax depth\z@ \kern-0.4pt\relax
         \else \vrule height\z@ depth\!chreventmarkdepth
         \fi
         \kern-0.4pt\relax
       \fi  
       \setbox0\vbox{%
         \if!chreventdate
           \hbox{#2}%
         \fi
         \hbox{%
          \ifdim\!chrperiodeventtextwidth > \z@ 
            \vbox {%
             \hsize\!chrperiodeventtextwidth #3%
            }%
          \else #3%
          \fi 
         }%
       }%
      \begingroup\dimen@\dimexpr\dp0+\ht0+2pt\relax
      \dimen@i\dimexpr\dimen@-\!chreventmarkdepth\relax
      \if!chreventlocationup
        \ifdim \dimen@i >\!chrskipbefore \global\!chrskipbefore\dimen@i \fi
      \else
        \ifdim \dimen@ >\!chrskipafter \global\!chrskipafter\dimen@ \fi
      \fi
      \endgroup
    }%
\fi\fi\fi}%
%
%
%
%
%
%
%
\!chrverif\def\setupchronoevent{\def\@@string@a{event}\!chrtraiteoneargument\dosetupchronoeventandperiode}%
\!chrverif\def\dosetupchronoeventandperiode[#1]#2{\if!chronearg
\def\@@string@a{#1}\fi \!chr@parcoursoptions#2,\end}%
%
%STOPCHRONOLOGY
%
%
\!chr@verif\newdimen\!chrstopwidth
\!chrverif\def\!chrstopcenteralign{\!chrstopwidth\dimexpr(\hsize-\!chrwidth)/2\relax}%
\!chrverif\def\!chrstopleftalign{\!chrstopwidth\z@}%
\!chrverif\def\!chrstoprightalign{\!chrstopwidth\dimexpr\hsize-\!chrwidth\relax}%
%
\!chrverif\def\stopchronology{\goodbreak
\ifcsname !chrstop\!chr@align align\endcsname
  \csname !chrstop\!chr@align align\endcsname
\else\!chrstopwidth\z@
\fi 
\vskip\!chrskipbefore
\moveright\!chrstopwidth\box\!chrflechebox
\vskip\!chrskipafter
\endgroup\bigskip}%
%
\!chr@verif\newif\if!chrverifdefines
\!chrverif\def\!chrverifdefines{%
 \ifcsname chrono\@@string@a\endcsname
   \!chrverifdefinesfalse \immediate\write16{Attention : macro \expandafter\noexpand\csname chrono\@@string@a\endcsname deja definie.}%
   \expandafter\!gobble 
 \else
   \!chrverifdefinestrue
   \expandafter\!chrverifdefines@ux
 \fi}%
\!chrverif\def\!chrverifdefines@ux{\expandafter\def\csname chrono\@@string@a\endcsname}%
%
%
%DEFINECHRONOEVENT
%
%
\!chrverif\def\definechronoevent#1{%
\def\@@string@a{#1}%
\!chrverifdefines{%
\expandafter\expandafter\expandafter\!chrtraitingargvirgule\expandafter\expandafter\expandafter{\csname !chr#1defaultoptions\endcsname}{!chr@event}%
\!chrtraiteoneargument\dochronoevent}%
\if!chrverifdefines
  \expandafter\def\csname !chr#1defaultoptions\endcsname{barre=true, icon=\relax,%
  markdepth=10pt, textstyle=\relax, mark=true,%
  date=true, datesseparation=\space, conversionmonth=true,%
  datestyle=\relax, datesstyle=\relax, year=true,%
  iconheight=0.5\!chrheight, ifcolorbox=true, colorbox=white,%
  textwidth=\relax}%
\fi
\ifnexttoken[{\!chr@defineorsetupoptions}{}}%
%
%
%DEFINECHRONOPERIODE
%
%
\!chrverif\def\definechronoperiode#1{%
\def\@@string@a{#1}%
\!chrverifdefines{%
\expandafter\expandafter\expandafter\!chrtraitingargvirgule\expandafter\expandafter\expandafter{\csname !chr#1defaultoptions\endcsname}{!chr@period}%
\!chrtraiteoneargument\dochronoperiode}%
\if!chrverifdefines
  \expandafter\def\csname !chr#1defaultoptions\endcsname{textdepth=15pt, dates=true,%
  color=\!chrperiodedef@ultcolor, datesstyle=\relax,%
  startdate=true, stopdate=true, textstyle=\relax,%
  dateselevation=0pt, ifcolorbox=true,%
  colorbox=white, bottomdepth=0pt, topheight=\!chrheight, box=false,%
  textwidth=\relax}%
\fi
\ifnexttoken[{\!chr@defineorsetupoptions}{}}%
%
%pour modifier les valeurs par d\'efaut
%
\!chrverif\def\!chr@defineorsetupoptions[#1]{%
\!chr@parcoursoptions#1,\end
}%
%
\!chrverif\def\!chr@parcoursoptions#1,{\!chr@replaceoptions#1,=\end,\ifnexttoken\end \!gobble \!chr@parcoursoptions}%
\!chrverif\def\!chr@replaceoptions#1=#2,{%
\ifx#2\end\relax
\else
  \def\@@string@f{}%
  \def\@@string@c{#1}\def\@@string@d{#2}%
  \expandafter\let\expandafter\@@string@@b\csname !chr\@@string@a defaultoptions\endcsname
  \expandafter\!chr@replaceoptionsaux\@@string@@b,\end%
  \expandafter\let\csname !chr\@@string@a defaultoptions\endcsname\@@string@f
  \expandafter\!gobblethree
\fi}%
%
\!chrverif\def\!chr@replaceoptionsaux#1,{\!chr@replaceoptions@ux#1,=\end,\ifnexttoken\end\!gobble\!chr@replaceoptionsaux}%
\!chrverif\def\!chr@replaceoptions@ux#1=#2,{%
\ifx#2\end\relax
\else
  \def\@@string@e{#1}% 
  \ifx\@@string@c\@@string@e
    \expandafter\def\expandafter\@@string@f\expandafter{\@@string@f , #1=}%
    \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@@string@f\expandafter\expandafter\expandafter{\expandafter\@@string@f\@@string@d}%
  \else 
    \expandafter\def\expandafter\@@string@f\expandafter{\@@string@f , #1=#2}%
  \fi
  \expandafter\!gobblethree
\fi
}%
%
%
\!chr@verif\newcount\!chrgraduationcount
\!chr@verif\newcount\!chrgraduationcount@ux
\newif\if!chrgradu@tionevent \!chrgradu@tioneventtrue
\!chrverif\def\chronograduation{\!chrtraitetwoargument\dochronograduation}%
\!chrverif\def\dochronograduation[#1][#2]#3{%
\if!chrtwoarg
  \def\@@string@a{#2}%
  \def\@@string@b{#1}\def\@@string@c{event}%
  \def\@@string@d{periode}%
  \ifx\@@string@b\@@string@c 
    \!chrgradu@tioneventtrue 
  \else
    \ifx\@@string@b\@@string@d 
      \!chrgradu@tioneventfalse
    \else 
    	\def\@@string@e{}\unless\ifx\@@string@b\@@string@e\immediate\write16{chronosys : style #1 non défini ligne \number\inputlineno}\fi
    \fi
  \fi 
\else \def\@@string@a{#1}%
\fi
\!chrgraduationcount\!chrstartyear
\if!chrgradu@tionevent
  \loop
    \advance\!chrgraduationcount#3%
    \ifnum\!chrgraduationcount<\!chrstopyear 
      \expandafter\chrono!!eventgradu@tion
      \expandafter[\@@string@a]{\number\!chrgraduationcount}{}%
  \repeat
\else 
  \def\@@string@e{startdate=true,}%
  \expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@@string@e\expandafter\expandafter\expandafter{\expandafter\@@string@e\@@string@a}%
  \expandafter\chrono!!periodegradu@tion\expandafter[\@@string@e]{\number\!chrgraduationcount}{#3}{}%
  \restartchronoperiodecolor
  \loop 
    \advance\!chrgraduationcount#3%
    \ifnum\!chrgraduationcount<\!chrstopyear
       \!chrgraduationcount@ux\numexpr\!chrgraduationcount-#3\relax \expandafter\chrono!!periodegradu@tion\expandafter[\@@string@a]{\number\!chrgraduationcount@ux}{\number\!chrgraduationcount}{}%
  \repeat
\fi}%
%
\!chrverif\def\setupchronograduation{\!chrtraiteoneargument\dosetupchronograduation}%
\!chrverif\def\dosetupchronograduation[#1]{%
\if!chronearg
  \def\@@string@b{#1}\def\@@string@c{event}\def\@@string@d{periode}%
  \ifx\@@string@b\@@string@c 
    \!chrgradu@tioneventtrue 
  \else
    \ifx\@@string@b\@@string@d 
      \!chrgradu@tioneventfalse
    \fi
  \fi 
\fi
\if!chrgradu@tionevent 
  \def\@@string@a{[!!eventgradu@tion]}%
\else \def\@@string@a{[!!periodegradu@tion]}%
\fi
\expandafter\setupchronoevent\@@string@a}%
%
\definechronoevent{event}%
\definechronoevent{!!eventgradu@tion}[markdepth=5pt,barre=false, ifcolorbox=false]%
\definechronoperiode{periode}%
\definechronoperiode{!!periodegradu@tion}[dateselevation=-10pt,%
startdate=false, ifcolorbox=false]%
%
\endinput
%
%
